Orbit spaces of Weyl groups acting on compact tori: a unified and explicit polynomial description

The Weyl group of a crystallographic root system has a nonlinear action on the compact torus. The orbit space of this action is a compact basic semi-algebraic set. We present a polynomial description of this set for the Weyl groups of type A, B, C, D and G. Our description is given through a polynomial matrix inequality. The novelty lies in an approach via Hermite quadratic forms and a closed formula for the matrix entries. The orbit space of the nonlinear Weyl group action is the orthogonality region of generalized Chebyshev polynomials. In this polynomial basis, we show that the matrices obtained for the five types follow the same, surprisingly simple pattern. This is applied to the optimization of trigonometric polynomials with crystallographic symmetries.

==> section3_symmetricpolynomialsandroots_backup.tex <==
\section{Symmetric polynomial systems}
\label{section:symmetricpolynomialsandroots}
\setcounter{equation}{0}

In order to give a polynomial description for the $\TTorus$--orbit space of a Weyl group, our first step is to study solutions of symmetric systems. We do this, because the symmetric group $\mathfrak{S}_n$ is a subgroup of all Weyl groups of $\RootA$, $\RootB$, $\RootC$, $\RootD$ and $\RootG[2]$. Thus symmetric systems play an essential role in \Cref{section_proofA,section_proofBCD,section_proofG}. We aim to characterize those systems that have all their solutions in the compact torus $\TTorus^n$.

%In this section, the univariate polynomial ring is denoted by $\Rt$. The univariate ring of Laurent polynomials is denoted by $\Rx=\R[x,x^{-1}]$.

\subsection{Solutions in $\TTorus^n$}

For $1\leq i \leq n$, the \textbf{$i$--th elementary symmetric function} in $n$ indeterminates is
\begin{equation}\label{DefinitionESP}
\sigma_i(y_1,\ldots,y_n) = \sum_{\substack{J \subseteq \{1 ,\ldots, n\} \\ \mbox{with } \vert J \vert = i }} \, \prod_{j\in J} y_j \in\R[y_1,\ldots,y_n].
\end{equation}
We shall be confronted with the following two types of polynomial systems in unknown $y_1,\ldots,y_n$.
\[
\begin{array}{clcl}
\mathrm{(I)}	&	\sigma_i(y_1			,\ldots,y_n				)	&=&	(-1)^i\,c_i \tbox{for} 1\leq i \leq n \tbox{with} c_1,\ldots,c_n\in\C \\
\mathrm{(II)}	&	\sigma_i(y_1+y_1^{-1}	,\ldots,y_n+y_n^{-1}	)	&=&	(-1)^i\,c_i \tbox{for} 1\leq i \leq n \tbox{with} c_1,\ldots,c_n\in\R
\end{array}
\]
The goal is to determine, whether all solutions $y=(y_1,\ldots,y_n)\in\C^n$ of system $\mathrm{(I)}$, respectively system $\mathrm{(II)}$, are contained in $\TTorus^n$.

\begin{lemma}\label{Correspondence2S}~
\begin{enumerate}
\item The map
\[
\begin{array}[t]{ccl}
\C^*	&	\to		&	\C,\\
 x		&	\mapsto	&	( x+ x^{-1})
\end{array}
\]
is surjective and the preimage of $[-2,2]$ is $\TTorus$.
\item System $\mathrm{(I)}$ always has a solution $y\in\C^n$. It is is unique up to permutation of coordinates.
\item System $\mathrm{(II)}$ always has a solution in $y\in(\C^*)^n$. It is is unique up to permutation and inversion of coordinates.
\end{enumerate}
\end{lemma}
\begin{proof}
\emph{1.} For $r\in\C$, consider the univariate polynomial $p:=x^2-r\,x+1$. Then $0$ is not a root of $p$ and $p=0$ if and only if $r=x+x^{-1}$, that is, $r$ is in the image of the map. If $r\in [-2,2]$, then $p$ has discriminant $(r/2)^2-1\leq 0$ and its two roots are $ x, \overline{x} = x,x^{-1} = r/2 \pm \mathrm{i}\,\sqrt{1-(r/2)^2}\in\TTorus$. On the other hand, for $x\in\TTorus$, we have $ x +  x^{-1}=x+\overline{ x} = 2\,\Re( x) \in [-2,2]$.

\emph{2.} By Vieta's formula, a solution of system $\mathrm{(I)}$ is the vector of roots of a polynomial with coefficients given by the right hand side of system $\mathrm{(I)}$. Since $\C$ is algebraically closed, the statement follows.

\emph{3.} By \emph{1.}, we can write the roots $r_1,\ldots,r_n$ of the polynomial with coefficients given by the right hand side of system $\mathrm{(II)}$ as $r_i=y_i+y_i^{-1}$ for some $y\in (\C^*)^n$. Then $y$ is a unique solution of $\mathrm{(II)}$ up to permutation and inversion.
\end{proof}

From now on, we speak of \emph{the} solution of system $\mathrm{(I)}$, respectively $\mathrm{(II)}$.

\begin{proposition}\label{SolutionsSystemII}
For $c_1,\ldots,c_n \in\R$, the solution of system $\mathrm{(II)}$ is contained in $\TTorus^n$ if and only if all the roots of the univariate polynomial
\[
	x^n+c_1\,x^{n-1}+\ldots+c_{n-1}\,x+c_n
\]
are contained in $[-2,2]$.
\end{proposition}
\begin{proof}
Let $p:=x^n+c_1\,x^{n-1}+\ldots+c_n$ be the univariate polynomial with roots $r_1,\ldots, r_n\in\C$. If $y\in(\C^*)^n$ is the solution of system $\mathrm{(II)}$, then for all $1\leq i\leq n$, $ y_i+ y_i^{-1}$ is a root of $p$ by Vieta's formula. Applying \Cref{Correspondence2S} yields $ y\in\TTorus^n$ if and only if $r_1,\ldots, r_n\in[-2,2]$.
\end{proof}

The \textbf{Chebyshev polynomial of the first kind} associated to $\ell\in\N$ is the unique univariate polynomial $T_\ell$ with $T_\ell((x+x^{-1})/2)=(x^\ell+x^{-\ell})/2$. For $0\neq p\in\Rt$ or $\Ct$, denote by $\coeff(x^\ell,p)$ the coefficient of the monomial $x^\ell$ in $p$ for $0\leq \ell \leq \deg(p)$.

\begin{proposition}\label{SolutionsSystemI}
For $c_1,\ldots,c_{n-1}\in\C$ with $\overline{c_i}=(-1)^n \,c_{n-i}$ and $c_0:=(-1)^n  \,c_n:=1$, the solution of system $\mathrm{(I)}$ is contained in $\TTorus^n$ if and only if all the roots of the univariate polynomial
\[
	T_n(x) + d_1\,T_{n-1}(x) + \ldots + d_{n-1} \, T_1(x) + \dfrac{d_n}{2} \, T_0(x)
	\tbox{with}
	d_{\ell}=\sum_{i=0}^\ell \overline{c_i}\,c_{\ell-i} \in \R
\]
are contained in $[-1,1]$.
\end{proposition}
\begin{proof}
By Vieta's formula, the solution of system $\mathrm{(I)}$ is contained in $\TTorus^n$ if and only if all the roots of the univariate polynomial $p:=x^n+c_1\,x^{n-1}+\ldots+c_n$ are contained in $\TTorus$.

The roots of $p$ are nonzero, because $p(0)=c_n=(-1)^n \neq 0$. We fix another univariate polynomial $\tilde{p}:=x^n+\overline{c_1}\,x^{n-1}+\ldots+\overline{c_n}$. Since $\tilde{p}(x) = (-x)^n\,p(x^{-1})$, the roots of $p\tilde{p}$ are the union of the roots of $p$ and their inverses. Especially, all the roots of $p\tilde{p}$ are contained in $\TTorus$ if and only if the roots of $p$ are. The coefficients of $p\tilde{p}$ satisfy
\[
	\coeff(x^\ell,p\tilde{p})	
=	\sum\limits_{i=0}^\ell 	c_{n-i} \, \overline{c_{n-\ell+i}}
=	\sum\limits_{i=0}^\ell \overline{c_{i}} \, c_{\ell-i}
=	\begin{cases}
			\sum\limits_{i=0}^\ell \coeff(x^{n-i},\tilde{p}) \, \coeff(x^{n-\ell+i},p)	=	\coeff(x^{2n-\ell},p\tilde{p})	\\
		 	\sum\limits_{i=0}^{\lfloor (\ell-1)/2 \rfloor} \underbrace{(\overline{c_i}\,c_{\ell-i} +  \overline{c_{\ell-i}}\,c_i)}_{\in\R} +
		\begin{cases}
			c_{\ell/2}\,\overline{c_{\ell/2}},	&	\ell \mbox{ even}\\
			0,									&	\ell \mbox{ odd}
		\end{cases}
		\in	\R
	\end{cases}
\]
for $0\leq \ell\leq n$. Thus, $\coeff(x^\ell,p\tilde{p})=\coeff(x^{2n-\ell},p\tilde{p})=d_\ell\in\R$ and %$p\tilde{p}$ is palindromic with real coefficients. Now, 
we can write
\[
	p\tilde{p}
=	\sum\limits_{\ell=1}^{n}	d_{n-\ell} (x^{n+\ell}+x^{n-\ell}) + d_n
=	2  x^n \left( \sum\limits_{\ell=1}^{n}	d_{n-\ell} T_\ell\left(\dfrac{x+x^{-1}}{2}\right) + \dfrac{d_n}{2} T_0\left(\dfrac{x+x^{-1}}{2}\right) \right)
=:	2 x^n g\left(\dfrac{x+x^{-1}}{2}\right).
\]
With \Cref{Correspondence2S}, we see that $x\in\TTorus$ is a root of $p\tilde{p}$ if and only if $(x+x^{-1})/2\in [-1,1]$ is a root of $g$.
\end{proof}

\subsection{Characterization of real roots via Hermite quadratic forms}

Let $p,q\in\Rt$ be univariate polynomials. The multiplication by $q$ in the $\R$--algebra $\Rt/\langle p \rangle$ is the homomorphism 
\[
m_q:
\begin{array}[t]{ccl}
\Rt/\langle p \rangle	&	\to		&	\Rt/\langle p\rangle , \\
f + \langle p \rangle	&	\mapsto	&	q \, f + \langle p \rangle .
\end{array}
\]
By \cite[Chapter 2, Proposition 4.2]{cox05}, for $q_1,q_2\in\Rt$, we have
\begin{equation}\label{MultiplicationMapRelations}
m_{q_1+q_2}=m_{q_1}+m_{q_2} \tbox{and}  m_{q_1\,q_2}=m_{q_1}\circ m_{q_2} .
\end{equation}

If $p=x^n+c_1\,x^{n-1}+\ldots+c_{n-1}\,x+c_n$, then the matrix of $m_x$ in the basis $\{1,x,\ldots,x^{n-1}\}$ of $\Rt/\langle p \rangle$ is the companion matrix
\begin{equation}\label{equation_CompMatrix}
\begin{bmatrix}
0		&			&	0		&	-c_n	\\
1		&	\ddots	&			&	\vdots	\\
		&	\ddots	&	0		&	-c_2	\\
0		&			&	1		&	-c_1	
\end{bmatrix}
\end{equation}
of $p$, because $x\,x^i=x^{i+1}$ for $0\leq i\leq n-2$ and $x\,x^{n-1} = x^n\equiv-c_1\,x^{n-1}-\ldots-c_{n-1}\,x-c_n \mbox{  mod  } \langle p \rangle$.

On the other hand, the univariate Chebyshev polynomials of the first kind up to degree $n-1$ also form a basis $\{T_0,T_1,\ldots,T_{n-1}\}$ of $\Rt/\langle p \rangle$. If $p=T_n+d_1\,T_{n-1}+\ldots+d_{n-1}\,T_1+d_n/2 \, T_0\in\Rt$ and $n\geq 3$, then the matrix of $m_x$ in this basis is
\begin{equation}\label{equation_CompMatrixChebyshev}
\begin{bmatrix}
0	&	1/2	&			&			&	0	&	-d_n/4		\\
1	&	0	&	\ddots	&			&		&	-d_{n-1}/2	\\
	&	1/2	&	\ddots	&	\ddots	&		&	\vdots			\\
	&		&	\ddots	&	\ddots	&	1/2	&	-d_3/2 		\\
	&		&			&	\ddots	&	0	&	(1-d_2)/2	\\
0	&		&			&			&	1/2	&	-d_1/2 
\end{bmatrix},
\end{equation}
where the rows and columns are indexed by $T_0,T_1,\ldots,T_{n-1}$. The entries in the columns originate from the recurrence formula $x\,T_0=T_1$ and $2\,x\,T_j=T_{j+1}+T_{j-1}$ for $1\leq j\leq n-1$. Especially,
\[
	2\,x\,T_{n-1}	=	T_n + T_{n-2}	\equiv	-d_1\,T_{n-1}+(1-d_2)\,T_{n-2}-d_3\,T_{n-3}-\ldots-d_{n-1}\,T_1-d_n/2\,T_0  \tbox{mod} \langle p \rangle
\]
yields the last column.

\begin{example}\label{Example_PalindromicPoly}
Let $p=x^3-c\,x^2+\overline{c}\,x-1\in\Ct$ with $c\in\C$. Following the proof of \Cref{SolutionsSystemI}, we consider the palindromic polynomial $p\tilde{p}\in\Rt$ with
\begin{align*}
	&	\,\dfrac{ 1}{2 x^{3}} \, p(x) \tilde{p}(x) \\
=	&	\,\dfrac{ 1}{2 x^{3}} \, \left((x^6+1)-(c+\overline{c})(x^5+x)+(c\,\overline{c}+c+\overline{c})(x^4+x^2)-\dfrac{c^2+\overline{c}^2+2}{2}\,x^3\right)\\
=	&	\,\dfrac{x^3+x^{-3}}{2}-(c+\overline{c})\,\dfrac{x^2+x^{-2}}{2}+(c\,\overline{c}+c+\overline{c})\,\dfrac{x+x^{-1}}{2}-\dfrac{c^2+\overline{c}^2+2}{2} \\
=	&	\,T_3\left(\dfrac{x+x^{-1}}{2}\right)-(c+\overline{c})\,T_2\left(\dfrac{x+x^{-1}}{2}\right)+(c\,\overline{c}+c+\overline{c})\,T_1\left(\dfrac{x+x^{-1}}{2}\right)-\dfrac{c^2+\overline{c}^2+2}{2}\,T_0\left(\dfrac{x+x^{-1}}{2}\right)\\
=	&	\,g\left(\dfrac{x+x^{-1}}{2}\right).
\end{align*}
The matrix of the multiplication by $x$ in $\Rt/\langle g \rangle$ in the basis of Chebyshev polynomials is
\begin{align*}
\begin{bmatrix}
0	&	1/2	&	(c^2+\overline{c}^2+2)/4				\\
1	&	0	&	(1-c\,\overline{c}-c-\overline{c})/2	\\
0	&	1/2	&	(c+\overline{c})/2
\end{bmatrix}
\in\R^{3\times 3}
\end{align*}
and all the roots of $p$ are in $\Image$ if and only if all the roots of $g$ are in $[-1,1]$.
\end{example}

To characterize univariate polynomials with roots in $[-2,2]$, respectively $[-1,1]$, we can now use the next statement, which is essentially Sylvester's version for Sturm's theorem for Hermite quadratic forms.

\begin{theorem}\label{HermiteCharacterization}
Let $p\in \Rt$ be of degree $n$ and $q \in \Rt$. Then all the roots of $p$ are contained in $S(q):=\{ x \in\R \,\vert\, q(x) \geq 0 \}$ if and only if the Hermite quadratic form
\[
	H(p,q):\begin{array}[t]{rcl}
	\Rt/\langle p \rangle	& 	\to		&	\R , \\
	f+\langle p \rangle		&	\mapsto	&	\trace (m_{q\,f^2})
	\end{array}
\]
is positive semi--definite.
\end{theorem}
\begin{proof}
Let $H\in\R^{n\times n}$ be the symmetric matrix associated to $H(p,q)$ for a fixed basis of $\Rt/\langle p \rangle$. Denote by $N_+$, respectively $N_-$, the number of strictly positive, respectively negative, eigenvalues of $H$, including their multiplicities. Then the rank and the signature of $H(p,q)$ are
\[
\begin{array}{rcrcl}
N_+ + N_-	& = &	\mathrm{Rank}(H(p,q))	& = &	\vert\{  x\in\C \, \vert\, p(x) =0 ,\, q( x) \neq 0 \}\vert ,	\\
N_+ - N_-	& = &	\mathrm{Sign}(H(p,q))	& = &	\underbrace{\vert\{  x\in \R \, \vert \,p(x)=0,\, q( x) > 0 \}\vert}_{=:n_+} \, - \, \underbrace{\vert\{  x\in \R \, \vert \, p(x)=0 ,\, q( x) < 0 \}\vert}_{=:n_-},
\end{array}
\]
see for example \cite[Theorem 4.57]{roy13} or \cite[Chapter 2, Theorem 5.2]{cox05}.

If all the roots of $p$ are contained in $S(q)$, then $n_-=0$, and thus
\[
	N_+ + N_-
=	\mathrm{Rank}(H(p,q))
=	\mathrm{Sign}(H(p,q))
=	n_+
=	N_+ - N_-.
\]
Hence, $N_-=0$ and all eigenvalues of $H$ are nonnegative, that is, $H(p,q)$ is positive semi--definite.

For the converse, assume that $H(p,q)$ is positive semi--definite. Then $N_-=0$ and
\[
	N_+
=	\mathrm{Sign}(H(p,q))
=	n_+-n_-\leq \mathrm{Rank}(H(p,q))
=	N_+,
\]
that is, $ n_+ - n_- = \mathrm{Rank}(H(p,q))$. On the other hand, $\mathrm{Rank}(H(p,q)) \geq n_+ + n_-$. Hence, $n_-=0$ and $\mathrm{Rank}(H(p,q)) = n_+$ implies that all the roots of $p$ are real and contained in $S(q)$.
\end{proof}

As corollaries, we obtain explicit characterizations for solutions of symmetric polynomial systems in $\TTorus^n$.

\begin{corollary}\label{Corollary_SolutionsSystemI}
Let $n\geq 3$. For $c_1,\ldots,c_n \in\C$ with $\overline{c_i}=(-1)^n \,c_{n-i}$ for $1\leq i \leq n-1$ and $c_0:=(-1)^n  \,c_n:=1$, the solution of system $\mathrm{(I)}$ is contained in $\TTorus^n$ if and only if the matrix $H\in\R^{n\times n}$ with entries
\begin{align*}
H_{ij}	&=	\trace(C^{i+j-2}-C^{i+j}) , \tbox{where}\\
C		&=	
\begin{bmatrix}
0	&	1/2	&			&			&	0	&	-d_n/4		\\
1	&	0	&	\ddots	&			&		&	-d_{n-1}/2	\\
	&	1/2	&	\ddots	&	\ddots	&		&	\vdots			\\
	&		&	\ddots	&	\ddots	&	1/2	&	-d_3/2 		\\
	&		&			&	\ddots	&	0	&	(1-d_2)/2	\\
0	&		&			&			&	1/2	&	-d_1/2 
\end{bmatrix}
\in\R^{n\times n} \tbox{and} d_{\ell}=\sum_{i=0}^\ell c_i\,\overline{c_{\ell-i}}\tbox{for} 1\leq \ell\leq n,
\end{align*}
is positive semi--definite.
\end{corollary}
\begin{proof}
$H$ is the matrix associated to the Hermite quadratic form $H(p,q)$ from \Cref{HermiteCharacterization} with $q = 1 - x^2 $ in the basis $\{1,x,x^2,\ldots,x^{n-1}\}$. Indeed, by \Cref{MultiplicationMapRelations}, the entries of the associated matrix are
\[
	\trace(m_{q\,x^{i-1}\,x^{j-1}})
=	\trace(m_{x^{i+j-2}-x^{i+j}})
=	\trace(m_x^{i+j-2}-m_x^{i+j})
\]
for $1\leq i,j\leq n$. Since the trace is independent of the basis for $\Rt/\langle p \rangle$, we can consider the matrix of $m_x$ in the basis of univariate Chebyshev polynomials of the first kind, which according to \Cref{equation_CompMatrixChebyshev} is $C$. The statement now follows from \Cref{SolutionsSystemI}.
\end{proof}

\begin{corollary}\label{Corollary_SolutionsSystemII}
For $c_1,\ldots,c_n \in\R$, the solution of system $\mathrm{(II)}$ is contained in $\TTorus^n$ if and only if the matrix $H\in\R^{n\times n}$ with entries
\begin{align*}
H_{ij}	&=	\trace(4\,C^{i+j-2}-C^{i+j}) , \tbox{where}\\
C		&=	
\begin{bmatrix}
0		&	\cdots	&	0		&	-c_n\phantom{_{-2}}\\
1		&			&	0		&	-c_{n-1}\\
		&	\ddots	&			&	\vdots\\
0		&			&	1		&	-c_1\phantom{_{-2}}
\end{bmatrix}\in \R^{n\times n},
\end{align*}
is positive semi--definite.
\end{corollary}
\begin{proof}
The proof is analogous to the one of \Cref{Corollary_SolutionsSystemI} with $q = 4 - x^2 $, \Cref{equation_CompMatrix} and \Cref{SolutionsSystemII}.
\end{proof}

%In our examples, we will characterize $H\succeq 0$ via the coefficients of the characteristic polynomial to give a proper visualization.

%\begin{proposition}\label{MatrixPSDCriterion}
%\cite[Theorem 4.58]{roy13} Let $A\in\R^{n\times n}$ be a symmetric matrix with characteristic polynomial
%\[
%	\det(x\,I_n-A) = x^n + \sum\limits_{i=1}^{n} (-1)^{i}\,a_i\,x^{n-i}\in\Rt.
%\]
%Then $A$ is positive semi--definite if and only if  $a_i \geq 0$ for all $1\leq i \leq n$.
%\end{proposition}

\clearpage
